In-Context Principle Learning from Mistakes

In-context learning (ICL, also known as few-shot prompting) has been the standard method of adapting LLMs to downstream tasks, by learning from a few input-output examples. Nonetheless, all ICL-based approaches only learn from correct input-output pairs. In this paper, we revisit this paradigm, by learning more from the few given input-output examples. We introduce Learning Principles (LEAP): First, we intentionally induce the model to make mistakes on these few examples; then we reflect on these mistakes, and learn explicit task-specific "principles" from them, which help solve similar problems and avoid common mistakes; finally, we prompt the model to answer unseen test questions using the original few-shot examples and these learned general principles. We evaluate LEAP on a wide range of benchmarks, including multi-hop question answering (Hotpot QA), textual QA (DROP), Big-Bench Hard reasoning, and math problems (GSM8K and MATH); in all these benchmarks, LEAP improves the strongest available LLMs such as GPT-3.5-turbo, GPT-4, GPT-4 turbo and Claude-2.1. For example, LEAP improves over the standard few-shot prompting using GPT-4 by 7.5% in DROP, and by 3.3% in HotpotQA. Importantly, LEAP does not require any more input or examples than the standard few-shot prompting settings.

==> sections/broader.tex <==


\section{Broader Impact}
This paper presents work that aims to advance the field of Machine Learning by presenting a method that allows \llms to learn from their own mistakes.
The potential of \llms to learn to correct their behaviors from past mistakes can significantly improve their capability without human-in-the-loop. 
This ability has many potential societal consequences, most notably the opportunity for LLMs to self-improve across a wide range of tasks where their initial performance may be lacking

==> sections/object_counting_example.tex <==
% \begin{figure}[t]
% \small
% \begin{analysisbox}[Object Counting (\bbh)]

% \textbf{Question:} I have a flute, a piano, a trombone, four stoves, a violin, an accordion, a clarinet, a drum, two lamps, and a trumpet. How many musical instruments do I have? \\
% \textbf{Task Principles:} \hl{
% % To improve future responses, it is important to carefully consider the quantity of each item when counting. 
% % ... Each individual item should be counted separately, regardless of whether they are the same type. ...
% The response should be directly related to the user's query or statement. Irrelevant information can confuse the user and detract from the overall quality of the response...
% } \\
% \textbf{Few-shot CoT:} Let's think step by step. We first identify the musical instruments on the list and include their quantity in parentheses: - flute (1) - piano (1) - trombone (1) - \mistake{stoves (4)} - violin (1) - accordion (1) - clarinet (1) - drum (1) - \mistake{lamps (2)} - trumpet (1) Now, let's add the numbers in parentheses: 1 + 1 + 1 + \mistake{4} + 1 + 1 + 1 + 1 + \mistake{2} + 1 = \mistake{14}. So the answer is \boxed{14}. \xmark \\
% \textbf{\llfb Response:} Let's think step by step. We first identify the musical instruments on the list and include their quantity in parentheses: - flute (1) - piano (1) - trombone (1) - violin (1) - accordion (1) - clarinet (1) - drum (1) - trumpet (1) Now, let's add the numbers in parentheses: \correct{1 + 1 + 1 + 1 + 1 + 1 + 1 + 1 = 8}. So the answer is \boxed{8}. \cmark
% \end{analysisbox}
% \caption{An example from the Object Counting task in \bbh. The learned principle is \hl{highlighted}, along with the \mistake{mistake} in \cotp  and the \correct{correct} reasoning generated by \ours.
% }
% \label{fig:analysis:objectcounting}
% % \vspace{-5mm}
% \end{figure}

==> tables/bbh_results_gpt4.tex <==
\begin{table}
\centering
\begin{tabular}{p{5cm}>{\centering\arraybackslash}p{2cm}>{\centering\arraybackslash}p{2cm}>{\centering\arraybackslash}p{2cm}>{\centering\arraybackslash}p{2.5cm}}
\toprule
Dataset                                     & \makecell{\cotp} & \makecell{LLL} & \makecell{HLL} & Winner \\
\midrule
                     boolean\_expressions &                  96.8 &                  \textbf{98.0} &                            97.6 &           \llfb \\
                        causal\_judgement &        \textbf{73.26} &                          72.73 &                           72.73 &            \cotp \\
                      date\_understanding &                  90.0 &                  \textbf{91.2} &                            90.0 &           \llfb \\
                       disambiguation\_qa &                  85.6 &                  \textbf{86.0} &                            85.2 &           \llfb \\
                          dyck\_languages &         \textbf{56.8} &                           56.8 &                            54.0 &            \cotp \\
                        formal\_fallacies &                  81.6 &                  \textbf{84.0} &                            81.6 &           \llfb \\
                        geometric\_shapes &                  54.4 &                           57.2 &                   \textbf{58.8} &           \hlfb \\
                              hyperbaton &                  98.0 &                  \textbf{99.2} &                            98.8 &           \llfb \\
          logical\_deduction\_five\_objects &                  85.2 &                  \textbf{85.6} &                            84.4 &           \llfb \\
         logical\_deduction\_seven\_objects &                  56.8 &                           58.4 &                   \textbf{59.6} &           \hlfb \\
         logical\_deduction\_three\_objects &         \textbf{99.2} &                           98.8 &                            98.8 &            \cotp \\
                    movie\_recommendation &                  90.4 &                           91.6 &                   \textbf{92.0} &           \hlfb \\
                multistep\_arithmetic\_two &                  93.2 &                  \textbf{94.0} &                            92.4 &           \llfb \\
                                navigate &                  98.0 &                  \textbf{98.4} &                            98.4 &           \llfb \\
                         object\_counting &                  98.8 &                  \textbf{99.2} &                            99.2 &           \llfb \\
                     penguins\_in\_a\_table &        \textbf{97.26} &                          96.58 &                           96.58 &            \cotp \\
         reasoning\_about\_colored\_objects &         \textbf{95.2} &                           91.2 &                            94.0 &            \cotp \\
                              ruin\_names &                  87.6 &                  \textbf{89.6} &                            87.6 &           \llfb \\
     salient\_translation\_error\_detection &         \textbf{68.8} &                           67.2 &                            67.2 &            \cotp \\
                                  snarks &                 89.89 &                          89.33 &                  \textbf{91.01} &           \hlfb \\
                    sports\_understanding &                  94.4 &                  \textbf{95.2} &                            94.4 &           \llfb \\
                      temporal\_sequences &        \textbf{100.0} &                          \textbf{100.0} &                           \textbf{100.0} &            \cotp \\
  tracking\_shuffled\_objects\_five\_objects &        \textbf{100.0} &                          \textbf{100.0} &                           \textbf{100.0} &            \cotp \\
 tracking\_shuffled\_objects\_seven\_objects &        \textbf{100.0} &                          \textbf{100.0} &                            98.8 &            \cotp \\
 tracking\_shuffled\_objects\_three\_objects &        \textbf{100.0} &                          \textbf{100.0} &                           \textbf{100.0} &            \cotp \\
                             web\_of\_lies &        \textbf{100.0} &                          \textbf{100.0} &                           \textbf{100.0} &            \cotp \\
                            word\_sorting &                  94.4 &                           94.0 &                   \textbf{95.6} &           \hlfb \\
\bottomrule
\end{tabular}
\caption{\textbf{\bbh Results:} Comparative performance results on various \bbh datasets using \gptf, highlighting the efficacy of the vanilla \cotp prompts alone and when augmented with Low-Level Feedback (LLL) and High-Level Feedback (HLL). One  of the variants of our method helps across 17 out of 27 tasks, will LLL outperforming \cotp and high-level feedback in 11 out of 27 datasets.}

\label{tab:results:bbh:gpt4}
\end{table}



==> tables/math_results_llama2_chat.tex <==
\begin{table}[h]
% TODO: Remove if we are short of space
% \renewcommand{\arraystretch}{1.2}
% \footnotesize
\caption{\textbf{Math Results}: Comparative performance results on MATH and GSM8K using \llama. We test across different variations of \texttt{Llama-2-70B-Chat} models and Claude. The augmented low-level feedback and high-level feedback win over traditional CoT in most cases.}
\label{tab:math_llama2}
% \setlength\tabcolsep{5pt}
\centering
\begin{tabular}{p{1.5cm}>{\centering\arraybackslash}p{3cm}>{\centering\arraybackslash}p{2.5cm}>{\centering\arraybackslash}p{2.5cm}>{\centering\arraybackslash}p{2.5cm}>{\centering\arraybackslash}p{2cm}>{\centering\arraybackslash}p{2cm}}
% {lcccccccccccc}
\toprule
& & \makecell{CoT} & \makecell{LO-FB} & \makecell{HL-FB} \\
\midrule
\multirow{2}{*}{GSM8K} & Llama-2 Critic & \textbf{52.5} & 50.6 & 47.0\\
 & GPT-4 Critic & \textbf{52.5} & 49.8 & 51.0\\
\midrule
\multirow{2}{*}{MATH} & Llama-2 Critic & \textbf{16.2} & 13.8 & 14.2 \\
& GPT-4 Critic & \textbf{16.2} & 12.9 & 13.8 \\
\bottomrule 
\end{tabular}
\end{table}

